Nash Equilibria on (Un)Stable Networks

In response to a change, individuals may choose to follow the responses of their friends or, alternatively, to change their friends. To model these decisions, consider a game where players choose their behaviors and friendships. In equilibrium, players internalize the need for consensus in forming friendships and choose their optimal strategies on subsets of k players - a form of bounded rationality. The k-player consensual dynamic delivers a probabilistic ranking of a game's equilibria, and, via a varying k, facilitates estimation of such games. Applying the model to adolescents' smoking suggests that: (a.) the response of the friendship network to changes in tobacco price amplifies the intended effect of price changes on smoking, (b.) racial desegregation of high-schools decreases the overall smoking prevalence, (c.) peer effect complementarities are substantially stronger between smokers compared to between non-smokers. (d.) the magnitude of the spillover effects from small scale policies targeting individuals' smoking choices are roughly double compared to the scale of these policies.

==> 01_literature_old.tex <==
\subsection{Related literature}

The empirical models in \cite{Nakajima2007} and \cite{Mele2017} inspired the proposed framework. \cite{Nakajima2007} studies peer effects abstracting from friendships and \cite{Mele2017} obtains large network asymptotics of a model with link formation only. The approaches in these papers are fundamentally compatible so these models can be unified in a joint model, as in \cite{hsieh2014social}, \cite{Boucher2016} and \cite{hsieha2016network}. Compared to existing frameworks, including \cite{CabralesCalvoArmengolZenou2011} and \cite{CanenTrebbiJackson2016}, I departure from purely non-cooperative formulations of individuals' decision problem. More specifically, the proposed solution concept embeds the necessity for consensus for forming a relationship (\citealp{Jackson_Wolinsky_1996}).%\footnote{Another important difference with \cite{Boucher2016} who also recognizes the possibility of multiplicity. The approach there is to select a particular equilibrium as opposed to resort to adaptive dynamic as equilibrium weighting tool.} %Importantly, the proposed formulation of individuals' decision problem is general and can found both statistical and non-statistical approaches for prediction. 

A handful of theoretical papers consider (broadly related) adaptive link dynamics or model both network formation along with other choices potentially affected by the network (See \citealp{JacksonWatts2002,goyal_vega-redondo_05,Cabrales2011,Hiller2012,KonigTessoneZenou2014nestedness,Baetz2014,LageraasSeim2016strategic}). For example \cite{KonigTessoneZenou2014nestedness} obtain a characterization, later generalized by \cite{LageraasSeim2016strategic}, of the Nash equilibria in our model as nested split graphs---graphs where nodes' neighborhoods have strict hierarchical structures, i.e. a node's neighborhood contains the neighborhoods of all nodes with lower degrees. Similar results are obtained by \cite{Hiller2012} in the context of $2$-player stable networks.\footnote{An analogous  characterization of the family of NE$k$SN should be of independent interest. Given the focus of this paper, I leave this for another occasion.}\footnote{In similar settings \cite{JacksonWatts2002} and \cite{goyal_vega-redondo_05} obtain conditions under which the risk-dominant or the efficient action prevails when they analyze similar dynamic processes (as opposed to the equilibrium networks).} Importantly, the theoretical frameworks available, are meant to provide focused insights into isolated features of networks and deliver sharp predictions, but are not easily adapted for the purposes of estimation.%
\footnote{A typical approach is to focus the analysis on a particular equilibrium as opposed to discussing all equilibria. Multiplicity of equilibria reflects the possibility of network and behavioral externalities which is an indispensable feature of our settings.} 

Potential function representation as a dimensionality reduction tool is  widely used in (algorithmic) game theory, computer science and in economics of networks for processes on fixed networks, for processes of link formation and, more recently, for combined processes, e.g. \cite{foster_young_90}, \cite{blume_03b}, \cite{JacksonWatts2002},  \cite{Nakajima2007}, \cite{BramoulleKrantonDAmours2014}, \cite{BourlesBramoullePerez-Richet2017}, \cite{Mele2017}, \cite{Boucher2016}, \cite{hsieh2014social}, \cite{hsieha2016network}.%
\footnote{Congestion games were the first class of games exhibiting this property (Beckmann, McGuire and Winsten, 1956; Rosenthal, 1973). Monderer and Shapley (1996) recognize that congestion games are instances of games with potential, propose several notions of potential functions for games in strategic form, and obtain a characterization of potential games.} 
In the proposed framework, the role of the potential function is to justify the gravitation of a family of adaptive dynamics around equilibria of the link/behavior game. This study also suggest a direction for addressing the poor statistical properties of those models.\footnote{This is an important point for the implementation of those models. For more background, see the discussion in \cite{BhamidiBrestlerSly_2011} and \cite{ArunJackson2016}.}

Econometric models of networks and actions are proposed in \cite{goldsmith2013social} and \cite{hsieh2014social} where the decisions to form friendships influence the decision to engage in a particular activity. The focus of their research, however, is not on policy analysis nor on accounting for the possible endogenous response of the friendship network to changing the decision environment. Thus, they are able to abstract from the converse feedback from actions to friendship formation and, also, to avoid the equilibrium microfoundations of a strategic model and an explicit treatment of the possibility for multiplicity. In contrast, the framework proposed in \cite{Boucher2016} is microfounded as a particular equilibrium in a non-cooperative model of friendships and behaviors. %\footnote{Multiplicity in our settings makes the model intractable and, more importantly, deteriorates the statistical power of model's predictions.}
Related work by \cite{hsieha2016network} propose a two-stage estimation procedure, with an application to R and D, which relies on conditional independence of links delivered by abstracting from link externalities. \cite{auerbach2016identification} obtains identification results within large network asymptotics which also rely on conditional independence of links. While the assumptions leading to conditional independence present a convenience, these limit the scope for studying peer effects, in addition ruling out externalities in the network formation.\footnote{It is important to realize that network economics owes its appeal namely because networks conceptualize so naturally situations with externalities, so ruling these out in essence defies the use of network economics.} Finally, there are recent contributions to the econometrics literature which focus on link formation, though these are not easily extendable to include action choice as well.\footnote{See \cite{Sheng2014structural}, \cite{ArunJackson2016}, \cite{Leung2014random}, \cite{dePaulaRichardsTamer2014identification}, \cite{Graham2014econometric}, \cite{Menzel2015strategic} and the reviews in \cite{Arun2015econometrics,dePaula2016Econometrics,Bramoulle2016Oxford}.}

The theoretical analysis in \cite{Jackson2016Paradox} argues that variability in individuals' popularity (degree in a social network) leads to biased perceptions for the social norm which in turn leads to higher levels of activities compared to a situation when there is no variability in individuals' popularity.\footnote{This increase is further amplified if the most popular individuals are those with the highest proclivity for extreme behaviors.} Although the model in this paper is different in that individuals choose their friends and I exploit different information assumptions, one of my counterfactual experiments hints to such amplification mechanisms (in quite different settings) where as a result of the endogenous response of the social network to a price increase the intended effects on the overall smoking are amplified.

The empirical analysis of friendship networks and smoking behaviors lends support to a host of results which are related to the large body of empirical work on social interactions and teen risky behaviors. Typically, empirical studies on peer effects either lack data on friendship network or take the friendship network as given.\footnote{See, for example, \cite{LiuPatacchiniZenou2014}, who distinguish between local aggregate and local average peer effects, and the references therein.}
 Also the approaches range from models that directly relate an individual's choices to mean characteristics of his peer groups\footnote{See \cite{powell_tauras_ross_05}, \cite{ali_dwyer_09}, and the references therein.} to models with elaborate equilibrium micro-foundations, such as those in \cite*{BrockDurlauf2001a,BrockDurlauf2007,Krauth2005b,Calvo-ArmengolPatacchiniZenou2009}. In terms of estimates, this paper makes the first step in explaining how not accounting for the response of these social network (e.g. as a result of lack of data) could bias the estimates.\footnote{It is difficult, if not impossible, to account the empirical contributions of the large literature on peer effects and teen risky behaviors. For a small sample of papers obtaining estimates of peer effects see \cite{ChaloupkaHenry1997}, \cite{ali2009estimating} and the references in \cite[Surgeon General's Report]{CDCSurgeonGeneral2000}.}
Similarly, this paper pioneers a mechanism capable of explaining the role of the school composition, or more generally the determinants of the social fabric, on the overall teen risky behaviors. The possibility of such a role was theorized by \cite{graham2014complementarity} and experimentally discovered by \cite{CarrellSacerdoteWest2013}.%
\footnote{It is important to recognize that this study has limitations. The presence of unobservables which affect both individuals' propensity to smoke and also the friendship decisions, in principle, could influence the model's predictions (See \cite{Manski1993} and the discussion in \cite{Blume_etal2015Review}.) While the model can be augmented to accommodate an extension along these lines, identification of model's parameters becomes delicate and frequentist and Bayesian perspectives differ substantially on this issue. Since I do not want to exploit the disagreement between those perspectives, I discuss this point only briefly and leave it for future research.}

==> 95_noncooperative_foundations.tex <==
\newpage
\section{NE$k$SN the outcome of a sub-game perfect Nash equilibrium}
The NE$k$SN outcome can arise from a sub-game perfect Nash equilibrium of a two-stage game where in the first stage agents express interest of being in a relationship and on the second stage agents confirm their interest. The outcome of being in a (mutual) relationship presumes that both parties have expressed interest in the first stage or if one party has expressed interest on the first stage and the other party has consented to that interest in the second stage. This is similar to the link-announcement game of \cite{Mayerson1977}.\footnote{See also \cite{CalvoArmengol2004} and \cite{BlochJackson2006}.} The novelty is the requirement for $k$-player perfection in the second stage.
  
\subsection{Setup}

Consider a two-stage game between $N$ players with preferences over the outcome given, as before, in (\ref{payoff}-\ref{payoff2}). In the first stage, each player expresses an interest to be in a relationship with another player, i.e. $g^i_{i,j}\in\{0,1\}$. After the first stage, relationships of mutual interest arise. 

After players see each other announcements, the players confirm their interest $g^c_{i,j}\in\{0,1\}$. In the presence of $k$-player perfection, each player is constrained on the second stage by confirming a profile of relationshpis which is at most $k-1$ link different from the first stage, i.e. $\sum |g^i_{ij}-g^c_{ij}| < k$. Finally, a relationship of mutual interest arise as $g_{ij}=g^c_{ij}*g^c_{ji}$.

if players choose armax cannot get k in the model. we need that there is locality. so arg max subject to constraint? distance to what --own play or proposed play?

==> 99_alternative.tex <==
\section{Additional empirical specifications}
This appendix replicates the empirical analysis with an alternative specification where the price of tobacco is substituted with log income. It is important to note that (a.) ...

\subsection{Sample statistics}
\input{tex_tables/table_sampleStats.tex}



\subsection{Counterfactual experiments}


\begin{table}[h]
\caption{Predicted Smoking Prevalence following Same-race Students Cap (specification including log income)}
\label{table:ctrf-schoolcomposition-income}
\begin{center}
\begin{tabular}{cccccccc}
Same-race & School & School & Overall & \multicolumn{4}{c}{p-val $H_0$} \\
cap ($\%$) & White  & Black   & ($Y$)  & $E[Y_{i}]=E[Y_{0}]$ & $E[Y_{i}]=E[Y_{i-1}]$ & $Y_{i}=Y_{0}$ & $Y_{i}=Y_{i-1}$\\ \hline \hline
0  & 27.0 &  6.7  & 16.8 & - & - & - & -  \\
10 & 25.0 &  8.1  & 16.7 & 0.12  & 0.12   & 0.12  & 0.12 \\
20 & 21.8 &  10.2  & 16.0 & 0.00  & 0.00   & 0.00  & 0.00 \\
30 & 20.6 &  11.0  & 15.8 & 0.00  & 0.18   & 0.00  & 0.33 \\
40 & 16.2 & 14.8  & 15.5 & 0.00  & 0.02   & 0.00  & 0.25 \\
50 & 15.1 & 15.4  & 15.2 & 0.00  & 0.02   & 0.00  & 0.01 \\ \hline
\end{tabular}
\end{center}
\fignotetitle{Note:} \fignotetext{A cap of $x\%$ same-race students is implemented with a swap of $(100-x)\%$ students. Columns 2, 3 and 4 show smoking prevalence. Columns 5 and 6 show the p value for the hypothesis of mean equality in overall smoking (t-test for mean equality; t-stat for unequal variances). Columns 7 and 8 show the p value for the hypothesis of equality in distribution of overall smoking (two-sample Kolmogorov-Smirnov test). Both test cannot reject the hypotheses for equal mean/equal distribution of the overall smoking for two cases: (a.) same-race cap 0\% and same-race cap 10\%, (b.) same-race cap 20\% and same-race cap 30\%, (c.) same-race cap 30\% and same-race cap 40\%, suggesting non-linear relation between school composition and overall smoking.}


\caption{Pairwise tests distribution overall smoking (specification including log income)}
\label{table:ctrf-schoolcomposition-income}
\begin{center}
\begin{tabular}{cccccccc}
Same-race & \multirow{2}{*}{0} & \multirow{2}{*}{10}&\multirow{2}{*}{20}&\multirow{2}{*}{30}&\multirow{2}{*}{40}&\multirow{2}{*}{50} \\
cap ($\%$) &  \\ \hline
0  & 1.00 (1.00) &     &   &   &   &    \\
10 & 0.12 (0.12) &  1.00 (1.00)  &   &    &     &     \\
20 & 0.00(0.00) &  0.00(0.00)  & 1.00 (1.00) &    &     &    \\
30 & 0.00(0.00) &  0.00(0.00) & 0.18(0.33) &1.00 (1.00)  &     &     \\
40 & 0.00(0.00) & 0.00(0.00)  & 0.00(0.01) & 0.02 (0.25)  &1.00 (1.00)  &     \\
50 & 0.00(0.00) & 0.00(0.00)  & 0.00(0.00) & 0.00 (0.00) & 0.02(0.01)   & 1.00 (1.00)  \\ \hline
\end{tabular}
\end{center}
\fignotetitle{Note:} \fignotetext{Each cell shows p value for the hypothesis of mean equality in overall smoking between a pair of scenarios (t-test for mean equality; t-stat for unequal variances). Each cell shows in parenthesis the p value for the hypothesis of equality in distribution of overall smoking (two-sample Kolmogorov-Smirnov test). For example both tests cannot reject the null when comparing equality in means (and equality in distributions) of overall smoking between scenarios same-race cap 0\% and same-race cap 10\% (p-value for both is $0.12$).}
\end{table}

\begin{table}[h]
\caption{Spillovers(specification including log income)}
\label{table:ctrf-spillovers-income}
\begin{center}
\begin{tabular}{ccccc}
\multirow{2}{*}{Campaign (\%)}  & \multirow{2}{*}{Smoking}  & \multicolumn{1}{c}{Predicted effect} & Actual & \multirow{2}{*}{Multiplier} \\
& & proportional & effect \\
 \hline \hline
-      & 44.0  & -      & -    & -   \\
1.0   & 40.0  & 0.4  & 3.2   & 7.4 \\
2.5  & 38.1  & 1.1    & 5.8   & 5.3 \\
5.0  & 34.6  & 2.1  & 9.4    & 4.2 \\
10.0 & 31.5  & 4.1  & 12.5  & 2.8 \\
20.0 & 25.5  & 8.2  & 18.4 & 2.1 \\
30.0 & 21.1  & 12.3 & 22.9 & 1.7 \\
50.0 & 11.3  & 20.5 & 32.7 & 1.5 \\ \hline
\end{tabular}
\end{center}
\fignotetitle{Note:} The first column lists the alternative attendance rates. The second and third columns display the smoking rate and the change in smoking rate respectively if the decrease would be proportional to the intervention, i.e. computes a baseline without peer effects. The last column computes the ratio between the percentage change in the number of smokers and the attendance rate.
\end{table}





\comments{
RESPONSE TO CHANGE IN INCOME IN PCT
[income_scenario(2:end) endog_nets_stats(2:end,1) policyeffect_endog, policyeffect_fixed, (policyeffect_endog-policyeffect_fixed), policyeffect_noPE, policyeffect_noPEv2]

ans =

    0.1000    0.3268    0.0130    0.0047    0.0083    0.0027    0.0006
    0.2000    0.3145    0.0253    0.0167    0.0086    0.0043    0.0025
    0.3000    0.3032    0.0366    0.0223    0.0143    0.0061    0.0044
    0.4000    0.2977    0.0421    0.0365    0.0056    0.0117    0.0076
    0.5000    0.2685    0.0713    0.0487    0.0226    0.0131    0.0087
    }

==> tex_tables/table_ctrfPrice_post_vs_meanPost.tex <==
% tex created by table_ctrfPrice_meanPosterior_vs_posterior.py 

    \begin{table}[htbp]
    \caption{The effect on smoking rate from changes in the price of tobacco}
    \label{table:ctrf-price}
    \begin{center}
    \begin{tabular}{ccccccccc}
    Price increase & Model  & Model  & Exog net & Exog net & No net data & No net data \\ \hline \hline
      20 &  2.5 &  2.5 &  2.2 &  2.2 &  1.3 &  1.3 \\ 
  40 &  4.7 &  4.9 &  4.2 &  4.2 &  2.6 &  2.6 \\ 
  60 &  6.9 &  7.2 &  6.1 &  6.2 &  3.9 &  3.9 \\ 
  80 &  8.7 &  9.4 &  7.9 &  8.1 &  5.1 &  5.2 \\ 
 100 & 10.3 & 11.3 &  9.4 &  9.9 &  6.2 &  6.4 \\ 
 120 & 11.8 & 13.1 & 10.9 & 11.6 &  7.4 &  7.6 \\ 
 140 & 13.1 & 14.8 & 12.3 & 13.1 &  8.4 &  8.8 \\ 
 160 & 14.3 & 16.3 & 13.5 & 14.5 &  9.5 &  9.9 \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} The first column shows proposed increases in tobacco prices in cents. 
    The average price of a pack of cigarettes is \$1.67 so that 20 cents is approximately 10\%. 
    The second through fourth columns show the predicted increase in the overall smoking (baseline 41\%) in ppt 
    from the full model, from the model when the friendship network is fixed, and 
    from the model when no social network data is available (i.e., $\phi_S=\phi_N=0$). 
    \end{table}
    

==> tex_tables/table_ctrfPrice_post_vs_meanPost2.tex <==
% tex created by table_ctrfPrice_meanPosterior_vs_posterior.py 

    \begin{table}[!h]
    \caption{Pairwise tests of the policy effects for different levels of price change}
    \label{table:ctrf-posteriorPrice-tests}
    \begin{center}
    \begin{tabular}{lccccccc}
    Policy & \multirow{2}{*}{20} & \multirow{2}{*}{40}&\multirow{2}{*}{60}&\multirow{2}{*}{80}&\multirow{2}{*}{100}&\multirow{2}{*}{120} \\
    level (dP)&  \\ \hline \hline
    20           & 1.00 (1.00) \\ 
40           & 0.00 (0.00) & 1.00 (1.00) \\ 
60           & 0.00 (0.00) & 0.00 (0.00) & 1.00 (1.00) \\ 
80           & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 1.00 (1.00) \\ 
100          & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 1.00 (1.00) \\ 
120          & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 1.00 (1.00) \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} \fignotetext{
    Each cell compares the policy effects for a pair of price changes.
    The two p-values are from testing a hypothesis of equal means and from testing a hypothesis of equal distributions
    (two-sample Kolmogorov-Smirnov test).}
    \end{table}
    

==> tex_tables/table_ctrfSchoolComposition_income.tex <==
% tex created by visuals_ctrfSchoolComposition_income.py 

    \begin{table}[h!]
    \caption{Predicted Smoking Prevalence following Same-race Students Cap}
    \label{table:ctrf-schoolcomposition}
    \begin{center}
    \begin{tabular}{cccc}
    Same-race & School & School & Overall \\
    cap ($\%$) & White  & Black   & \\ \hline \hline
      0 &  5.0 & 33.5 & 19.3 \\ 
 10 &  7.2 & 30.2 & 18.7 \\ 
 20 &  9.9 & 26.6 & 18.3 \\ 
 30 & 11.6 & 24.8 & 18.2 \\ 
 40 & 16.3 & 19.4 & 17.9 \\ 
 50 & 17.6 & 18.3 & 17.9 \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} \fignotetext{A cap of $x\%$ same-race students is implemented with a swap of $(100-x)\%$ students. 
    The last column shows the predicted changes in overall smoking under different same-race caps. 
    The policy induces statistically significant changes in the overall smoking as suggested by 
    the statistical tests in appendix D.}
    \end{table}
    

==> tex_tables/table_ctrfSchoolComposition_income_tests.tex <==
% tex created by visuals_ctrfSchoolComposition_income.py 

    \begin{table}[!h]
    \caption{Pairwise tests of the response of the overall smoking to same-race caps}
    \label{table:ctrf-schoolcomposition-tests}
    \begin{center}
    \begin{tabular}{cccccccc}
    Same-race & \multirow{2}{*}{0} & \multirow{2}{*}{10}&\multirow{2}{*}{20}&\multirow{2}{*}{30}&\multirow{2}{*}{40}&\multirow{2}{*}{50} \\
    cap ($\%$) &  \\ \hline \hline
      0 & 1.00 (1.00) \\ 
 10 & 0.00 (0.01) & 1.00 (1.00) \\ 
 20 & 0.00 (0.00) & 0.00 (0.00) & 1.00 (1.00) \\ 
 30 & 0.00 (0.00) & 0.00 (0.00) & 0.58 (0.47) & 1.00 (1.00) \\ 
 40 & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.00) & 1.00 (1.00) \\ 
 50 & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01) & 0.04 (0.03) & 0.68 (0.99) & 1.00 (1.00) \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} \fignotetext{Each cell examines the change in overall prevelance between a pair of scenarios (same-race caps).
    The two p-values are from testing a hypothesis of equal means and from testing a hypothesis of equal distributions
    (two-sample Kolmogorov-Smirnov test). 
    For example, both tests cannot reject the null (of equal means and equal distributions) 
    of the overall smoking between a same-race cap of 40\% and a same-race cap of 50\% (p-value $0.37 (0.95)$).
    For all other cases the policy induces statistically significant changes in the overall smoking.}
    \end{table}
    

==> tex_tables/table_ctrfSpills_extended.tex <==
% tex created by table_ctrfSpills.py 

    \begin{table}[!h]
    \caption{Spillovers}
    \label{table:ctrf-spillovers}
    \begin{center}
    \begin{tabular}{ccccccc}
    \multirow{2}{2cm}{Campaign size (\%)}  
    & \multirow{2}{2cm}{Predicted smoking} 
    & \multicolumn{4}{c}{Predicted effect}
    & \multirow{2}{*}{Multiplier} \\
    & & Model
    & Exog net
    & No net data
    & Prop    
    \\
     \hline \hline
    - & 42.1 & - & - & - & - & \\ 
   3& 39.6&  2.6&  2.0&  2.0&  1.3&  2.0 \\ 
   5& 38.2&  3.9&  3.1&  3.1&  2.1&  1.9 \\ 
  10& 34.6&  7.5&  5.9&  6.1&  4.2&  1.8 \\ 
  20& 28.7& 13.4& 10.7& 11.0&  8.4&  1.6 \\ 
  30& 23.5& 18.6& 14.9& 15.4& 12.6&  1.5 \\ 
  50& 15.1& 27.0& 21.9& 22.4& 21.1&  1.3 \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} The first and the second columns list the alternative attendance rates and the simulated smoking prevalences respectively.
    Columns three to six display the simulated decrease in overall smoking for different estimation scenarios:
        the full model, the model with exogenous (fixed) social network, the model with no social network data, and 
        the policy effect if it were (only) proportional to the intervention, i.e. a baseline without peer effects. 
        The last column computes the ratio between the percentage change in the number of smokers and the attendance rate.
        %Note that that attendance is random with respect to the smoking status of the students. 
        %If the campaign is able to target only students who are currently smokers, the spillover effects will be even larger.
    \end{table}
    

==> tex_tables/table_ctrfSpills_income.tex <==
% tex created by table_ctrfSpills.py 

    \begin{table}[!h]
    \caption{Spillovers}
    \label{table:ctrf-spillovers}
    \begin{center}
    \begin{tabular}{ccccc}
    \multirow{2}{*}{Campaign (\%)}  & \multirow{2}{*}{Smoking}  & \multicolumn{1}{c}{Predicted effect} & Actual & \multirow{2}{*}{Multiplier} \\
    & & proportional & effect \\
     \hline \hline
    - & 43.1 & - & - & \\ 
   3& 40.7&  1.3&  2.4&  1.9 \\ 
   5& 39.3&  2.2&  3.8&  1.8 \\ 
  10& 35.7&  4.3&  7.4&  1.7 \\ 
  20& 29.8&  8.6& 13.3&  1.5 \\ 
  30& 24.5& 12.9& 18.6&  1.4 \\ 
  50& 15.8& 21.5& 27.2&  1.3 \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} The first column lists the alternative attendance rates. The second and third columns display the smoking rate and the change in smoking rate respectively if the decrease would be proportional to the intervention, i.e. computes a baseline without peer effects. The last column computes the ratio between the percentage change in the number of smokers and the attendance rate. Note that that attendance is random with respect to the smoking status of the students. If the campaign is able to target only students who are currently smokers, the spillover effects will be even larger.
    \end{table}
    

==> tex_tables/table_ctrfSpills_income_extended.tex <==
% tex created by table_ctrfSpills.py 

    \begin{table}[!h]
    \caption{Spillovers}
    \label{table:ctrf-spillovers}
    \begin{center}
    \begin{tabular}{ccccccc}
    \multirow{2}{2cm}{Campaign size (\%)}  
    & \multirow{2}{2cm}{Predicted smoking} 
    & \multicolumn{4}{c}{Predicted effect}
    & \multirow{2}{*}{Multiplier} \\
    & & Model
    & Exog net
    & No net data
    & Prop    
    \\
     \hline \hline
    - & 43.1 & - & - & - & - & \\ 
   3& 40.7&  2.4&  2.6&  2.6&  1.3&  1.9 \\ 
   5& 39.3&  3.8&  4.0&  4.0&  2.2&  1.8 \\ 
  10& 35.7&  7.4&  7.8&  7.9&  4.3&  1.7 \\ 
  20& 29.8& 13.3& 13.8& 14.0&  8.6&  1.5 \\ 
  30& 24.5& 18.6& 19.0& 19.5& 12.9&  1.4 \\ 
  50& 15.8& 27.2& 27.3& 28.2& 21.5&  1.3 \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} The first and the second columns list the alternative attendance rates and the simulated smoking prevalences respectively.
    Columns three to six display the simulated decrease in overall smoking for different estimation scenarios:
        the full model, the model with exogenous (fixed) social network, the model with no social network data, and 
        the policy effect if it were (only) proportional to the intervention, i.e. a baseline without peer effects. 
        The last column computes the ratio between the percentage change in the number of smokers and the attendance rate.
        %Note that that attendance is random with respect to the smoking status of the students. 
        %If the campaign is able to target only students who are currently smokers, the spillover effects will be even larger.
    \end{table}
    

==> tex_tables/table_estimates_extended.tex <==
% tex created by table_estimates.py 

%\begin{table}[t!]
\begin{sidewaystable}
\begin{center}
\caption{Parameter estimates (posterior means)} \label{tab:estimates_extended}
\hspace*{-1cm}
\scalebox{0.8}{
\begin{tabular}{llccccccccc}
\hline \hline
\multicolumn{4}{c}{\textit{Utility of smoking}}  \\
   & Parameter   & No net data & Exog net & No PE & No link exter & No costs & No tri & $\phi_S=\phi_N$ & Model \\ \hline  1 &Baseline probability of smoking          &  $0.12^{***}$ &  $0.17^{***}$ &  $0.21^{***}$ &  $0.17^{***}$ &  $0.17^{***}$ &  $0.16^{***}$ &  $0.22^{***}$ &  $0.18^{***}$ \\ 
  2 &Price $\times 100$                       &    $-0.17^{}$ &    $-0.21^{}$ & $-0.61^{***}$ &   $-0.22^{*}$ &   $-0.24^{*}$ &    $-0.22^{}$ & $-0.32^{***}$ &   $-0.24^{*}$ \\ 
  3 &Mom edu (HS\&CO)$^{MP}$                  & $-0.04^{***}$ & $-0.05^{***}$ & $-0.05^{***}$ & $-0.05^{***}$ & $-0.05^{***}$ & $-0.05^{***}$ & $-0.06^{***}$ & $-0.05^{***}$ \\ 
  4 &HH smokes                                &  $0.11^{***}$ &  $0.13^{***}$ &  $0.16^{***}$ &  $0.13^{***}$ &  $0.13^{***}$ &  $0.13^{***}$ &  $0.15^{***}$ &  $0.14^{***}$ \\ 
  5 &Grade 9+$^{MP}$                          &  $0.18^{***}$ &  $0.16^{***}$ &  $0.24^{***}$ &  $0.18^{***}$ &  $0.17^{***}$ &  $0.18^{***}$ &  $0.16^{***}$ &  $0.16^{***}$ \\ 
  6 &Blacks$^{MP}$                            &  $-0.3^{***}$ &  $-0.3^{***}$ & $-0.35^{***}$ & $-0.31^{***}$ & $-0.31^{***}$ & $-0.31^{***}$ & $-0.34^{***}$ & $-0.31^{***}$ \\ 
  7 &$30\%$ of the school smokes$^{MP}$       &  $0.07^{***}$ &  $0.05^{***}$ &            -- &  $0.05^{***}$ &  $0.05^{***}$ &  $0.05^{***}$ &  $0.05^{***}$ &  $0.05^{***}$ \\ 

\\
\multicolumn{4}{c}{\textit{Utility of friendships}} \\
& Parameter   & No net data & Exog net & No PE & No link exter & No costs & No tri & $\phi_S=\phi_N$ & Model \\ \hline  8 &Baseline number of friends               &            -- &            -- &  $4.63^{***}$ &  $1.62^{***}$ &  $1.62^{***}$ &  $1.64^{***}$ &  $3.35^{***}$ &   $3.4^{***}$ \\ 
  9 &Different sex$^{MP\%}$                   &            -- &            -- & $-0.72^{***}$ & $-0.73^{***}$ & $-0.72^{***}$ & $-0.72^{***}$ & $-0.73^{***}$ & $-0.72^{***}$ \\ 
 10 &Different grades$^{MP\%}$                &            -- &            -- & $-0.89^{***}$ & $-0.86^{***}$ & $-0.85^{***}$ & $-0.86^{***}$ & $-0.89^{***}$ & $-0.89^{***}$ \\ 
 11 &Different race$^{MP\%}$                  &            -- &            -- &   $-0.33^{*}$ & $-0.24^{***}$ & $-0.37^{***}$ & $-0.34^{***}$ & $-0.26^{***}$ & $-0.39^{***}$ \\ 
 12 &Cost/Economy of scale                    &            -- &            -- & $-0.21^{***}$ &            -- &            -- &     $-0.0^{}$ & $-0.21^{***}$ & $-0.22^{***}$ \\ 
 13 &Triangles$^{MP\%}$                       &            -- &            -- &  $1.18^{***}$ &            -- &   $0.08^{**}$ &            -- &  $1.15^{***}$ &  $1.22^{***}$ \\ 
 14 &$\phi_{smoke}^{MP}$                      &            -- &  $0.04^{***}$ &            -- &  $0.05^{***}$ &  $0.05^{***}$ &  $0.04^{***}$ &  $0.05^{***}$ &  $0.05^{***}$ \\ 
 15 &$\phi_{nosmoke}^{MP}$                    &            -- &  $0.03^{***}$ &            -- &  $0.04^{***}$ &  $0.04^{***}$ &  $0.04^{***}$ &  $0.05^{***}$ &  $0.04^{***}$ \\ 

\\ \hline
\end{tabular}%
} %end scalebox
\end{center}
\fignotetitle{Note:} \fignotetext{MP stands for the estimated marginal probability in percentage points and MP$\%$ for estimated marginal probability in percent, relative to the baseline probability. The posterior sample contains $10^5$ simulations before discarding the first $20\%$. The shortest $90/95/99\%$ credible sets not including zero is indicated by $^{*}$/$^{**}$/$^{***}$ respectively.}
\end{sidewaystable}
%\end{table}


==> tex_tables/table_estimates_income.tex <==
% tex created by table_estimates.py 

\begin{table}[h]
\begin{center}
\caption{Parameter estimates (posterior means)} \label{tab:estimates}
\hspace*{-1cm}
\scalebox{0.8}{
\begin{tabular}{llcccccc}
\hline \hline
\multicolumn{4}{c}{\textit{Utility of smoking}}  \\
 & Parameter   & No net data & Exog net & No PE & Model \\ \hline  1 &Baseline probability of smoking          &  $0.13^{***}$ &  $0.17^{***}$ &  $0.24^{***}$ &  $0.21^{***}$ \\ 
  2 &Log income $\times 10$                   &   $1.0^{***}$ &  $0.99^{***}$ &  $1.07^{***}$ &  $1.03^{***}$ \\ 
  3 &Mom edu (HS\&CO)$^{MP}$                  & $-0.04^{***}$ & $-0.05^{***}$ & $-0.07^{***}$ & $-0.06^{***}$ \\ 
  4 &HH smokes                                &  $0.11^{***}$ &  $0.14^{***}$ &  $0.17^{***}$ &  $0.15^{***}$ \\ 
  5 &Grade 9+$^{MP}$                          &  $0.15^{***}$ &  $0.14^{***}$ &   $0.2^{***}$ &  $0.13^{***}$ \\ 
  6 &Blacks$^{MP}$                            & $-0.29^{***}$ &  $-0.3^{***}$ & $-0.37^{***}$ & $-0.32^{***}$ \\ 
  7 &$30\%$ of the school smokes$^{MP}$       &  $0.07^{***}$ &  $0.06^{***}$ &            -- &  $0.05^{***}$ \\ 

\\
\multicolumn{4}{c}{\textit{Utility of friendships}} \\
& Parameter   & No net data & Exog net & No PE & Model \\ \hline  8 &Baseline number of friends               &            -- &            -- &  $4.53^{***}$ &  $3.52^{***}$ \\ 
  9 &Different sex$^{MP\%}$                   &            -- &            -- & $-0.71^{***}$ & $-0.72^{***}$ \\ 
 10 &Different grades$^{MP\%}$                &            -- &            -- & $-0.89^{***}$ & $-0.88^{***}$ \\ 
 11 &Different race$^{MP\%}$                  &            -- &            -- & $-0.32^{***}$ & $-0.45^{***}$ \\ 
 12 &Cost/Economy of scale                    &            -- &            -- &  $-0.2^{***}$ & $-0.22^{***}$ \\ 
 13 &Triangles$^{MP\%}$                       &            -- &            -- &  $1.13^{***}$ &  $1.26^{***}$ \\ 
 14 &$\phi_{smoke}^{MP}$                      &            -- &  $0.05^{***}$ &            -- &  $0.06^{***}$ \\ 
 15 &$\phi_{nosmoke}^{MP}$                    &            -- &  $0.03^{***}$ &            -- &  $0.04^{***}$ \\ 

\\ \hline
\end{tabular}%
} %end scalebox
\end{center}
\fignotetitle{Note:} \fignotetext{MP stands for the estimated marginal probability in percentage points and MP$\%$ for estimated marginal probability in percent, relative to the baseline probability. The posterior sample contains $10^5$ simulations before discarding the first $20\%$. The shortest $90/95/99\%$ credible sets not including zero is indicated by $^{*}$/$^{**}$/$^{***}$ respectively.}
\end{table}


==> tex_tables/table_estimates_income_extended.tex <==
% tex created by table_estimates.py 

%\begin{table}[t!]
\begin{sidewaystable}
\begin{center}
\caption{Parameter estimates (posterior means)} \label{tab:estimates_extended}
\hspace*{-1cm}
\scalebox{0.8}{
\begin{tabular}{llccccccccc}
\hline \hline
\multicolumn{4}{c}{\textit{Utility of smoking}}  \\
   & Parameter   & No net data & Exog net & No PE & No link exter & No costs & No tri & $\phi_S=\phi_N$ & Model \\ \hline  1 &Baseline probability of smoking          &  $0.13^{***}$ &  $0.17^{***}$ &  $0.24^{***}$ &  $0.17^{***}$ &  $0.19^{***}$ &  $0.19^{***}$ &  $0.18^{***}$ &  $0.21^{***}$ \\ 
  2 &Log income $\times 10$                   &   $1.0^{***}$ &  $0.99^{***}$ &  $1.07^{***}$ &  $0.98^{***}$ &   $1.0^{***}$ &   $1.0^{***}$ &  $0.95^{***}$ &  $1.03^{***}$ \\ 
  3 &Mom edu (HS\&CO)$^{MP}$                  & $-0.04^{***}$ & $-0.05^{***}$ & $-0.07^{***}$ & $-0.05^{***}$ & $-0.05^{***}$ & $-0.05^{***}$ & $-0.05^{***}$ & $-0.06^{***}$ \\ 
  4 &HH smokes                                &  $0.11^{***}$ &  $0.14^{***}$ &  $0.17^{***}$ &  $0.14^{***}$ &  $0.14^{***}$ &  $0.14^{***}$ &  $0.14^{***}$ &  $0.15^{***}$ \\ 
  5 &Grade 9+$^{MP}$                          &  $0.15^{***}$ &  $0.14^{***}$ &   $0.2^{***}$ &  $0.15^{***}$ &  $0.15^{***}$ &  $0.14^{***}$ &  $0.15^{***}$ &  $0.13^{***}$ \\ 
  6 &Blacks$^{MP}$                            & $-0.29^{***}$ &  $-0.3^{***}$ & $-0.37^{***}$ & $-0.31^{***}$ & $-0.32^{***}$ & $-0.32^{***}$ & $-0.31^{***}$ & $-0.32^{***}$ \\ 
  7 &$30\%$ of the school smokes$^{MP}$       &  $0.07^{***}$ &  $0.06^{***}$ &            -- &  $0.06^{***}$ &  $0.05^{***}$ &  $0.05^{***}$ &  $0.06^{***}$ &  $0.05^{***}$ \\ 

\\
\multicolumn{4}{c}{\textit{Utility of friendships}} \\
& Parameter   & No net data & Exog net & No PE & No link exter & No costs & No tri & $\phi_S=\phi_N$ & Model \\ \hline  8 &Baseline number of friends               &            -- &            -- &  $4.53^{***}$ &  $1.61^{***}$ &  $1.61^{***}$ &  $1.63^{***}$ &  $3.38^{***}$ &  $3.52^{***}$ \\ 
  9 &Different sex$^{MP\%}$                   &            -- &            -- & $-0.71^{***}$ & $-0.71^{***}$ & $-0.72^{***}$ & $-0.72^{***}$ & $-0.72^{***}$ & $-0.72^{***}$ \\ 
 10 &Different grades$^{MP\%}$                &            -- &            -- & $-0.89^{***}$ & $-0.86^{***}$ & $-0.86^{***}$ & $-0.86^{***}$ & $-0.89^{***}$ & $-0.88^{***}$ \\ 
 11 &Different race$^{MP\%}$                  &            -- &            -- & $-0.32^{***}$ & $-0.38^{***}$ &    $-0.32^{}$ & $-0.37^{***}$ & $-0.39^{***}$ & $-0.45^{***}$ \\ 
 12 &Cost/Economy of scale                    &            -- &            -- &  $-0.2^{***}$ &            -- &            -- &     $-0.0^{}$ & $-0.21^{***}$ & $-0.22^{***}$ \\ 
 13 &Triangles$^{MP\%}$                       &            -- &            -- &  $1.13^{***}$ &            -- &   $0.08^{**}$ &            -- &  $1.17^{***}$ &  $1.26^{***}$ \\ 
 14 &$\phi_{smoke}^{MP}$                      &            -- &  $0.05^{***}$ &            -- &  $0.05^{***}$ &  $0.05^{***}$ &  $0.05^{***}$ &  $0.04^{***}$ &  $0.06^{***}$ \\ 
 15 &$\phi_{nosmoke}^{MP}$                    &            -- &  $0.03^{***}$ &            -- &  $0.04^{***}$ &  $0.04^{***}$ &  $0.04^{***}$ &  $0.04^{***}$ &  $0.04^{***}$ \\ 

\\ \hline
\end{tabular}%
} %end scalebox
\end{center}
\fignotetitle{Note:} \fignotetext{MP stands for the estimated marginal probability in percentage points and MP$\%$ for estimated marginal probability in percent, relative to the baseline probability. The posterior sample contains $10^5$ simulations before discarding the first $20\%$. The shortest $90/95/99\%$ credible sets not including zero is indicated by $^{*}$/$^{**}$/$^{***}$ respectively.}
\end{sidewaystable}
%\end{table}


==> tex_tables/table_fit_income.tex <==
% tex created by table_fit.py 

\begin{table}[h]
\caption{Model fit}
\label{table:fit}
\begin{center}
\begin{tabular}{lcc}
\hline \hline
\multicolumn{3}{c}{\textit{Selected moments}} \\
    Moment & Model & Data \\ \hline 
              Prevalence & 0.410 (0.408) & 0.408  \\ 
                 Density & 0.007 (0.005) & 0.005  \\ 
              Avg degree & 1.250 (0.966) & 0.973  \\ 
              Min degree & 0.275 (0.000) & 0.000  \\ 
              Max degree & 4.808 (4.568) & 5.308  \\ 
        $a_ig_{ij}a_j/n$ & 0.543 (0.253) & 0.256  \\ 
$(1-a_i)g_{ij}(1-a_j)/n$ & 0.400 (0.396) & 0.404  \\ 
           Two-paths$/n$ & 0.639 (0.490) & 0.501  \\ 
           Triangles$/n$ & 7.686 (0.023) & 0.066  \\ 

\\
\multicolumn{3}{c}{\textit{Mixing patterns}} \\ 
                      HI & 0.239 (0.231) & 0.236  \\ 
                     CHI & -0.300 (-0.299) & -0.303  \\ 
                     FSI & 0.665 (0.667) & 0.662  \\ 

\hline \\
\end{tabular}
\end{center}

\fignotetitle{Note:} 
\fignotetext{Columns Data and Model compare selected moments of the estimation sample with those of synthetic data 
generated by the estimated model. For the latter mean and median are reported (median in parentheses). 
Two-paths is defined as $\sum_{i>j} g_{ij}g_{il}(1-g_{il})$. Triangles is defined as $\sum_{i>j>l}g_{ij}g_{il}g_{il}$.
The Homophily index (HI), Coleman homophily index (CHI), and Freeman segregation index (FSI) 
are measures of the mixing patterns between students with the same smoking statuses (see also table \ref{table:fit_mixing}). 
For more details, see \cite{CurrariniJacksonPin2010} Definitions 1 and 2 in the supplemental appendix.}
\end{table} 


==> tex_tables/table_fit_income_mixing.tex <==
% tex created by table_fit.py 

\begin{table}[htbp]
\caption{Fit mixing matrix (model left, data right)}
\label{table:fit_mixing}
\centering
\begin{footnotesize}
\begin{tabular}{llcccc}
%\cmidrule{2-4} \morecmidrules \cmidrule{2-4}
  &  & \multicolumn{2}{c}{\axislabel{Nominee}}                                 & \multicolumn{2}{c}{\axislabel{Nominee}} \\
  \multirow{5}{*}{\rotatebox[origin=c]{90}{\axislabel{Nominator}}}
  &            & Smoker               & Nonsmoker                      & Smoker               & Nonsmoker           \\\cmidrule{2-6}
& Smoker   & \textbf{  65\% (56.6)} &   35\% (30.1) & \textbf{  63\% (52.1)} &   37\% (30.4)\\ 
 & Nonsmoker   &   29\% (30.1)& \textbf{   71\% (74.0)} &   29\% (30.4) & \textbf{   71\% (75.4)}
\\
\cmidrule{2-6}
\end{tabular}

\end{footnotesize}
%\fignotetitle{Source:} \fignotetext{The National Longitudinal Study of Adolescent Health (Add Health) - Wave I, 1994-95 school year (Estimation sample: $14$ schools, $1,125$ students, $21\%$ smokers).}
\end{table}


==> tex_tables/table_posterior_logIncome_tests.tex <==
% tex created by visuals_posteriorPrice_income.py 

    \begin{table}[!h]
    \caption{Pairwise tests of the posteriors for the (log) income parameter under different estimation scenarios}
    \label{table:ctrf-posteriorPrice-tests}
    \begin{center}
    \begin{tabular}{lccccccc}
    Estimation & \multirow{2}{*}{Model} & \multirow{2}{*}{Fixed net}&\multirow{2}{*}{No net data}&\multirow{2}{*}{No PE}&\multirow{2}{*}{No tri}&\multirow{2}{*}{No cost} \\
    scenarios &  \\ \hline \hline
    Model        & 1.00 (1.00) \\ 
Exog net     & 0.00 (0.00) & 1.00 (1.00) \\ 
No net data  & 0.00 (0.00) & 0.00 (0.00) & 1.00 (1.00) \\ 
No PE        & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 1.00 (1.00) \\ 

    \hline
    \end{tabular}
    \end{center}
    \fignotetitle{Note:} \fignotetext{
    Each cell compares the posterior distribution of the parameter (log) income between a pair of estimation scenarios.
    The two p-values are from testing a hypothesis of equal means and from testing a hypothesis of equal distributions
    (two-sample Kolmogorov-Smirnov test).}
    \end{table}
    

==> tex_tables/table_priors_income.tex <==
% tex created by table_priors_income.py 

\begin{table}[t]
\label{table:priors}
\begin{center}
\caption{Paramaters of the normal prior distributions}
\begin{tabular}{llccc}
\hline \hline
\multicolumn{4}{c}{\textit{Utility of smoking}}  \\
& Parameter &   Prior mean &   Prior std \\ \hline
  1 &Baseline probability of smoking          & 0.20   &   0.10 \\ 
  2 &Log income                               & 0.10   &   0.10 \\ 
  3 &Mom edu (HS\&CO)$^{MP}$                  & -0.05   &   0.05 \\ 
  4 &HH smokes                                & 0.10   &   0.10 \\ 
  5 &Grade 9+$^{MP}$                          & 0.20   &   0.20 \\ 
  6 &Blacks$^{MP}$                            & -0.20   &   0.20 \\ 
  7 &$30\%$ of the school smokes$^{MP}$       & 0.05   &   0.10 \\ 

\\
\multicolumn{4}{c}{\textit{Utility of friendships}} \\
& Parameter &   Prior mean &   Prior std \\ \hline
  8 &Baseline number of friends               & 3.00   &   2.00 \\ 
  9 &Different sex$^{MP\%}$                   & -0.70   &   0.50 \\ 
 10 &Different grades$^{MP\%}$                & -0.70   &   0.50 \\ 
 11 &Different race$^{MP\%}$                  & -0.50   &   0.50 \\ 
 12 &Cost/Economy of scale                    & 0.00   &   0.50 \\ 
 13 &Triangles$^{MP\%}$                       & 0.00   &   2.00 \\ 
 14 &$\phi^{MP}$                              & 0.05   &   0.05 \\ 

\hline
\end{tabular}
\label{table:descriptive_stats}
\end{center}
\fignotetitle{Note:} \fignotetext{All prior distributions are normals.}
\end{table}


==> tex_tables/table_sampleStats_100minus.tex <==
% tex created by table_descriptiveStats_saturatedSample.py 

\begin{table}[t]
\label{table:descriptive_stats}
\begin{center}
\caption{Descriptive Statistics for the estimation sample}
\begin{tabular}{lcccc}
\hline \hline
            &    Overall &          Min &       Max &     Median \\ \hline
Students    &        525 &          42 &         98 &         56 \\ 
Smoking     &       0.13 &        0.04 &       0.37 &        0.09 \\ 
Male        &       0.46 &        0.35 &       0.49 &        0.48 \\ 
Whites      &       0.75 &        0.00 &       0.99 &        0.95 \\ 
Blacks      &       0.17 &        0.00 &       0.97 &        0.00 \\ 
As-Hi-Ot    &       0.08 &        0.01 &       0.37 &        0.04 \\ 
Price       &     174.90 &      160.20 &     197.32 &      179.17 \\ 
Avg income  &      44.99 &       17.94 &      77.81 &       27.65 \\ 
Mom edu     &       0.85 &        0.73 &       0.95 &        0.90 \\ 
HH smokes   &       0.29 &        0.09 &       0.54 &        0.27 \\ 
Num friends  &       0.76 &        0.27 &       1.46 &        0.61 \\ 

\hline
\end{tabular}
\label{table:descriptive_stats}
\end{center}
\fignotetitle{Note:} \fignotetext{The final sample contains students from 8 high schools. Min, max, and median are reported at a school level.}
\end{table}

